2D Ego-Motion with Yaw Estimation using Only mmWave Radars via Two-Way weighted ICP

The interest in single-chip mmWave Radar is driven by their compact form factor, cost-effectiveness, and robustness under harsh environmental conditions. Despite its promising attributes, the principal limitation of mmWave radar lies in its capacity for autonomous yaw rate estimation. Conventional solutions have often resorted to integrating inertial measurement unit (IMU) or deploying multiple radar units to circumvent this shortcoming. This paper introduces an innovative methodology for two-dimensional ego-motion estimation, focusing on yaw rate deduction, utilizing solely mmWave radar sensors. By applying a weighted Iterated Closest Point (ICP) algorithm to register processed points derived from heatmap data, our method facilitates 2D ego-motion estimation devoid of prior information. Through experimental validation, we verified the effectiveness and promise of our technique for ego-motion estimation using exclusively radar data.

==> note.tex <==
Camera Calibration of Thermal-Infrared Stereo Vision System
pg199 맨 윗줄에 circluar patten detecton이 checker board patten 찾는것보다 더 정확하다고 설명되있음

총 실행시간(ms)라는 내용 넣기

1. target geometry 위치
    method의 하나의 subsection으로
 
2. related work의 범위
 알고리즘을 완성시키는데 필요한 논문들은 method에서 다루고 calibration 관련 논문만 소개하자.
 
 3. 첫 페이지 그림 배치
 개발한 타겟이 첫 페이지에 나와주는게 임팩트 있을것 같은데 구조가 조금 난잡해 지는 문제
 ->두 그림 하나로 합치자
 
 4. introduction에 왜 point 기반이 아닌 conic을 사용했는지에 대한 설명 필요

----------------------------------------------------------

동일 시간이 흘렀을때 캘판과 우리 target의 boundary 변화를 figure로 나타내자
 

==> result_table.tex <==
%\begin{table*}
%\resizebox{\linewidth}{!}{
%\begin{tabular}{c|c|cccc|c} 
%\hline
%\multirow{2}{*}{\textbf{Criteria}} & \multirow{2}{*}{\textbf{Approach}} &\multicolumn{4}{c|}{\textbf{Mulran Dataset}} & {\textbf{Oxford Dataset}}\\ 

% & & \textbf{DCC}  & \textbf{KAIST} & \textbf{Riverside} & \textbf{Sejong} & \textbf{2019-01-16 to 2019-01-18}\\ 
%\hline\hline
% & Raplace(Proposed) & \textbf{0.932} & \textbf{0.930} & \textbf{0.971} & \textbf{0.906} & %\textbf{0.949} \\
%\textbf{F1 Score} & Scan Context & 0.867 & 0.899 & 0.802 & 0.819 & 0.679\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx\\
%\cline{1-7}
%& Raplace(Proposed) & \textbf{0.978} & \textbf{0.984} & \textbf{0.995} & \textbf{0.969} & %\textbf{0.959} \\
%\textbf{AUC} & Scan Context & 0.952 & 0.978 & 0.915 & 0.929 & 0.773\\
%& PointNetVLAD & 0.xxx & 0.xxx & 0.xxx & 0.xxx & 0.xxx  \\

%\end{tabular}}
%\caption{Global Localization Results.}\label{tab:gl_result}
%\end{table*}

\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|ccc}
\multicolumn{2}{c}{\textbf{Dataset}}                                                    & \textbf{Method} & \textbf{AUC}   & \textbf{F1 Score} \\ \hline\hline
\multicolumn{1}{c|}{\multirow{12}{*}{MulRan}} & \multirow{3}{*}{DCC}       & ScanContext     & 0.952          & 0.867             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.978} & \textbf{0.932}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{KAIST}     & ScanContext     & 0.978          & 0.899    \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.984} & \textbf{0.930}             \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Riverside} & ScanContext     & 0.915          & 0.802             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\  
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.995} & \textbf{0.971}    \\ \cline{2-5} 
\multicolumn{1}{c|}{}                         & \multirow{3}{*}{Sejong}    & ScanContext     & 0.929          & 0.819             \\ 
\multicolumn{1}{c|}{}                         &                            & PointNetVlad    &                &                   \\
\multicolumn{1}{c|}{}                         &                            & RaPlace         & \textbf{0.969} & \textbf{0.906}    \\ \hline
\multicolumn{2}{c|}{\multirow{3}{*}{Oxford}}                     & ScanContext     & 0.773          & 0.679             \\  
\multicolumn{2}{c|}{}                                              & PointNetVlad    &                &                   \\ 
\multicolumn{2}{c|}{}                                          & RaPlace         & \textbf{0.959} & \textbf{0.949}    \\  \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}

==> result_table_comb.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cc|c|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset}}}                    & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Global Localization}}       \\
\multicolumn{2}{c|}{}                                                     &                                  & \multicolumn{1}{c}{\textbf{AUC}}   & \textbf{F1 Score} \\ \hline \hline
\multicolumn{1}{c|}{\multirow{8}{*}{MulRan}} & \multirow{2}{*}{DCC}       & SC                               & \multicolumn{1}{c}{0.952}          & 0.867             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.978}} & \textbf{0.932}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{KAIST}     & SC                               & \multicolumn{1}{c}{0.978}          & 0.899             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.984}} & \textbf{0.930}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Riverside} & SC                               & \multicolumn{1}{c}{0.915}          & 0.802             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.995}} & \textbf{0.971}    \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Sejong}    & SC                               & \multicolumn{1}{c}{0.929}          & 0.819             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.969}} & \textbf{0.906}    \\ \hline
\multicolumn{1}{c|}{\multirow{2}{*}{Oxford}} & \multirow{2}{*}{19-01-16}  & SC                               & \multicolumn{1}{c}{0.773}          & 0.679             \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.959}} & \textbf{0.949}    \\ \hline
\end{tabular}
}
\caption{Global Localization Results}\label{tab:gl_result}
\end{table}

==> result_table_pr.tex <==
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cc|c|cc}
\hline
\multicolumn{2}{c|}{\multirow{2}{*}{\textbf{Dataset}}}                    & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Single Session}}\\
\multicolumn{2}{c|}{}                                                     &                                  & \multicolumn{1}{c}{\textbf{AUC}}   & \textbf{F1 Score}\\ \hline \hline
\multicolumn{1}{c|}{\multirow{8}{*}{MulRan}} & \multirow{2}{*}{DCC}       & R-SC                               & \multicolumn{1}{c}{0.801}          & 0.679            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.843}} & \textbf{0.735}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{KAIST}     & R-SC                               & \multicolumn{1}{c}{0.819}          & \textbf{0.786}   \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.881}} & 0.781            \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Riverside} & R-SC                               & \multicolumn{1}{c}{0.944}          & 0.862            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.959}} & \textbf{0.897}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{Sejong}    & R-SC                               & \multicolumn{1}{c}{0.904}          & 0.830            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.924}} & \textbf{0.858}   \\ \hline
\multicolumn{1}{c|}{\multirow{4}{*}{Oxford}} & \multirow{2}{*}{19-01-16}  & R-SC                               & \multicolumn{1}{c}{0.545}          & 0.534            \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.595}} & \textbf{0.543}   \\ \cline{2-5}
\multicolumn{1}{c|}{}                        & \multirow{2}{*}{19-01-18}  & R-SC                               & \multicolumn{1}{c}{0.826}          & \textbf{0.773}   \\
\multicolumn{1}{c|}{}                        &                            & RP                               & \multicolumn{1}{c}{\textbf{0.827}} & 0.734            \\ \hline
\end{tabular}
}
\caption{Intra-session Place Recognition Results}\label{tab:pr_result}
\vspace{-5mm}
\end{table}
